Generalizability of Graph Neural Networks for Decentralized Unlabeled Motion Planning

Unlabeled motion planning involves assigning a set of robots to target locations while ensuring collision avoidance, aiming to minimize the total distance traveled. The problem forms an essential building block for multi-robot systems in applications such as exploration, surveillance, and transportation. We address this problem in a decentralized setting where each robot knows only the positions of its $k$-nearest robots and $k$-nearest targets. This scenario combines elements of combinatorial assignment and continuous-space motion planning, posing significant scalability challenges for traditional centralized approaches. To overcome these challenges, we propose a decentralized policy learned via a Graph Neural Network (GNN). The GNN enables robots to determine (1) what information to communicate to neighbors and (2) how to integrate received information with local observations for decision-making. We train the GNN using imitation learning with the centralized Hungarian algorithm as the expert policy, and further fine-tune it using reinforcement learning to avoid collisions and enhance performance. Extensive empirical evaluations demonstrate the scalability and effectiveness of our approach. The GNN policy trained on 100 robots generalizes to scenarios with up to 500 robots, outperforming state-of-the-art solutions by 8.6\% on average and significantly surpassing greedy decentralized methods. This work lays the foundation for solving multi-robot coordination problems in settings where scalability is important.

==> extra.tex <==
\section{Introduction}

The problem of unlabeled motion planning has applications in many different fields, such as search and rescue \pcite, surveillance \pcite, or any other task that can be done by a robot swarm. However, designing a controller for a swarm of robots to solve the unlabeled multi-agent motion planning problem has been shown to be hard, even when the swarm is homogeneous and the workspace contains simple polygonal obstacles \cite{solovey-amapf}. It follows that for more complex situations, it is impossible in polynomial time to create an analytic controller, centralized or decentralized, that solves the unlabeled multi-agent motion planning problem completely. However, it is possible to learn a heuristic to approximate a solution faster than a traditional algorithm could \cite{tolstaya-gnn-il}. We use this idea to develop a graph neural network-based algorithm that utilizes communication between agents to find an effective solution to the unlabeled motion planning problem.

Initially, we do not consider collisions or obstacles; instead, we focus on the simultaneous assignment and basic control problem. Specifically, imitation learning is done so that the GNN learns to solve the most basic version of the problem. Then, we use reinforcement learning to fine-tune the policy generated via imitation learning to maximize the reward obtained. We show that it is possible to learn a heuristic that outperforms other decentralized algorithms in terms of target coverage. Through fine-tuning done by reinforcement learning on the imitation learning algorithm, we can also discourage agents from colliding, improving the safety of the algorithm.

\section{Literature Review}

The ability to use solve decentralized robotics tasks using GNNs and supervised learning from a centralized algorithm was shown by \cite{tolstaya-gnn-il}. This is especially important in dynamic tasks, where the graph that describes the situation changes over time, crucially showing that graph neural networks can still be effective control solutions to these problems. GNNs are effective ways to solve problems of this nature due to the imposition of structure and the ability to represent communication between agents. The combination of imitation learning and GNNs can feasibly solve the labeled motion planning problem \cite{li-gnn-mapf}. By training using the data obtained by the online expert, the GNN was able to greatly outperform the known baseline, ORCA. We aim to improve upon this result by examining how a GNN based model can imitate an expert algorithm to solve the unlabeled motion planning problem. Additionally, we seek to create an algorithm that works in continuous-space, which is generally more complex than the discrete-space problems solved by other algorithms.

The unlabeled motion planning problem is similar to the coverage control problem where agents are placed in an importance density field with no information of the field a priori and seek to maximize the reward obtained by all agents. In both the coverage control problem and the unlabeled motion planning problem, the agents in the field do not have any information about the objectives (the importance density or the positions of the targets) before starting. Since GNNs have been successfully been applied to the coverage control problem, it is reasonable to expect that the same model can learn to solve the unlabeled motion planning problem utilizing the same principles \cite{gosrich-coverage-control}. Zhou et. al. has also shown the ability for a GNN to learn a complex decentralized task (target tracking) using a handcrafted vector to process each agent's surroundings \cite{zhou-target-tracking}. We create a similar vector to encode the positions of each agent's nearest neighbors and targets, as well as information about its own state.

[[We can use the fact that the order in which nearby agents and targets are observed to use Deep Sets, which process information in a manner that is permutation invariant \cite{zaheer-deep-sets}. Rivière et. al. shows that it is possible to learn a motion planning policy while using deep sets to process observations of nearby agents and targets. This suggests that we can simplify the model by using a small number of consistently-sized learned functions to process a theoretically infinite number of observations \cite{riviere-glas}. We will attempt to use deep sets in order to process information from neighbors and targets within a sensing radius. While past attempts to learn a solution to the unlabeled motion planning problem used a fixed number of sensed agents and targets, deep sets can create an embedding that involves many numbers of agents.]]

To improve the results obtained by imitation learning, reinforcement learning has been used to fine-tune a model pretrained using imitation. Ramrakhya et. al. showed this process to be effective when applied to the problem of object-goal navigation \cite{ramrakhya-pirlnav}. After pretraining the model, the fine-tuning was split into two phases: the critic learning phase, where the critic model is trained from the frozen IL policy, and the interactive learning phase, where the actor is unfrozen to improve the policy's performance from the pretrained stage. The idea of using reinforcement learning to supplement imitation learning has even be applied to multi-agent pathfinding \cite{damani-primal2}. (NOT TECHNICALLY; FIND A WAY TO PHRASE THIS CORRECTLY) In this case, environment randomization was also used to ensure that the neural network would be able to learn the optimal policy for a wide variety of situations. [[It has also been shown that a centralized critic function can be used to solve a problem using multi-agent reinforcement learning. The critic takes in as inputs the state of the environment and the actions of all agents in the environment, and since critics are not used during the execution of the model, the agents still solve the problem in a decentralized manner \cite{lowe-ma-rl}. It has also been suggested that the on-policy PPO algorithm can learn a more optimal policy than off-policy algorithms such as DDPG even though off-policy algorithms are seen as more sample efficient \cite{yu-mappo}. We can test this in the case of multi-agent motion planning by implementing both on-policy and off-policy algorithms and comparing their results.]] To optimize the policy and obtain desired results, we can use reward engineering techniques to find a reward function that will improve the policy obtained by imitation learning most efficiently. Peng et. al. suggests that a reward function that rewards the agent for performing the ideal action can result in better performance than a reward function that simply looks at the state \cite{peng-deepmimic}. Blumenkamp et. al. additionally demonstrated how reinforcement learning can be applied to agents that utilize GNN architectures to communicate with nearby agents \cite{blumenkamp-gnn-rl}. This research shows that it is possible to fuse GNNs and reinforcement learning to solve complex problems that cannot be solved by imitation learning approaches alone.

This work is the first example of a continuous-space multi-agent system being trained first using imitation learning and then finetuned through reinforcement learning. Additionally, we show that our algorithm experiences very little degradation in performance when it is applied to situations with many more agents than present in the training data. These results suggest that our algorithm is very scalable, which has not been seen in many other learned multi-agent motion planning algorithms.

\section{Principal Neighborhood Aggregation (PNA) vs. Summation Aggregation}

The original architecture uses summation in order to aggregate information from neighbors, so we also tested the principal neighborhood aggregation scheme. Specifically, we used all four operations of mean, standard deviation, minimum, and maximum as aggregators, concatenated the outputs (so that each agent had a node signal of size 512), and then fed them through a linear layer in order to convert them back to 128 channels. The results are shown in Figure \ref{fig:pna}. As we can see, the architecture that utilizes PNA performs marginal better than the original architecture, but a t-test would need to be used to determine the statistical significance of this improvement.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/pna.png}
    \caption{Reward over Time for the Original Architecture (blue) and PNA Architecture (orange)}
    \label{fig:pna}
\end{figure}

\section{Multi-Environment Training}

We also trained the architecture (using the summation aggregation) on multiple environments. The dataset comprises of 10 randomly generated episodes that uses the centralized policy. Instead of all of these episodes containing 100 agents and a field size of 100 square units, at the beginning of each episode, its number of agents and field size were each randomly chosen between 50, 100, and 200. This allowed the training set to be comprised of many different environments. The results of this training tested on different environments was compared with the original training scheme and is shown in Figures \ref{fig:mt-100-100}, \ref{fig:mt-50-50}, \ref{fig:mt-200-200}, \ref{fig:mt-50-200}, and \ref{fig:mt-100-400}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/mt-100-100.png}
    \caption{Reward over time when both training schemes are tested with 100 agents on a field size of 100}
    \label{fig:mt-100-100}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/mt-50-50.png}
    \caption{Reward over time when both training schemes are tested with 50 agents on a field size of 50}
    \label{fig:mt-50-50}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/mt-200-200.png}
    \caption{Reward over time when both training schemes are tested with 200 agents on a field size of 200}
    \label{fig:mt-200-200}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/mt-50-200.png}
    \caption{Reward over time when both training schemes are tested with 50 agents on a field size of 200}
    \label{fig:mt-50-200}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/mt-100-400.png}
    \caption{Reward over time when both training schemes are tested with 100 agents on a field size of 400}
    \label{fig:mt-100-400}
\end{figure}

\section{Multi-Scenario Training}

We developed various scenarios and trained the model on them. The original scenario on which all previous models were trained consisted of both the agents and the targets being placed uniformly around the field. We also created scenarios where the agents were normally distributed around 10 randomly placed points on the field, where the agents were uniformly distributed on the edge of a circle on the field, and where the agents were uniformly distributed in a smaller area in the center of the field. The first two scenarios, along with the uniform one, were considered "nice" scenarios. In all three of the additional scenarios, targets were still placed uniformly around the field. Figure \ref{fig:multi-scenario} compares the model when trained on only the uniform scenario, all of the "nice" scenarios, and all of the scenarios. The plot shows the results of all of these models tested on the uniform scenario.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/scenario_comparison_uniform.png}
    \caption{Reward over time of the models tested on multiple scenarios}
    \label{fig:multi-scenario}
\end{figure}

\section{Taps}

This was a small experiment to see what would happen as the number of filter taps used increases. We compared a GNN with 0 filter taps (which is just a neural network for each node), one with 2 filter taps, and one with 4 filter taps. The results are shown in Figure \ref{fig:taps}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/taps_comparison.png}
    \caption{Reward over time of the models with different numbers of filter taps}
    \label{fig:taps}
\end{figure}

\section{Future Endeavors}

Damian has come up with a complex-valued architecture that will allow for rotationally equivariant and invariant features. We plan on implementing this new architecture and comparing it with the original to see if the addition of rotational equivariance will improve the performance of the model.
